Calabi-Yau crystals in topological string theory

This thesis is concerned with a realisation of topological theories in terms of statistical models known as Calabi-Yau crystals. The thesis starts with an introduction and review of topological field and string theories. Subsequently several new results are presented. The main focus of the thesis is on the topological string theory. In this case crystal models correspond to three-dimensional partitions and their relations with the topological vertex theory and knot invariants are studied. Two-dimensional crystal models corresponding to topological gauge theories on ALE spaces are also introduced and analysed. Essential mathematical tools are summarised in appendices.

==> crystal-intro-old.tex <==
Topological string theories introduced in chapter \ref{chap-top-strings} are a very interesting area of research. Being simple enough to allow a computation of exact amplitudes, they exhibit a rich phenomena of the quantum world. An example of such a phenomenon is the open-closed duality, whose detailed understanding is believed to enhance our understanding not only of more complicated models, such as AdS/CFT correspondence, but also of QCD and quantum gravity. Topological string amplitudes constitute also a subset of superstring amplitudes and compute certain couplings in an effective supergravity theory. All these connections provide a strong motivation for studying topological string theories. 

The simplicity of topological strings does not actually mean the computation of their amplitudes is simple. A-model amplitudes we focus on in this thesis can be computed in a rigorous way in the Gromov-Witten theory, which is however a highly involved branch of mathematics and it provides answers only for particular Calabi-Yau target spaces. The physical method of the topological vertex introduced in section \ref{chap-top-vertex}, which is based on the open-closed duality and relation to Chern-Simons theory,  allows to solve topological strings on a wide class of toric geometries, although the results are quite complicated --- already a single topological vertex $C_{R_1 R_2 R_3}$ is a very non-trivial function of $q=e^{-g_s}$.

However, it turns out these topological A-model amplitudes for Calabi-Yau manifolds have a remarkable property --- they are reproduced by partition or generating functions of simple models of crystal melting known from statistical mechanics. This also allows to interpret toric Calabi-Yau manifolds as \emph{quantum manifolds} in terms of approprietly understood \emph{quantum geometry}, and in this context these crystal models are called \emph{Calabi-Yau crystals}. The equivalence with crystal generating functions reveals a remarkable simplicity and elegancy of the topological string partition functions which we are going to discuss in this chapter.

Crystal models related to Calabi-Yau manifolds are defined in terms of the so-called \emph{plane partitions}. There are two classes of these models. Firstly, the topological vertex amplitude $C_{R_1 R_2 R_3}$ can be interpreted as a certain generating function of plane partitions representing a single $\C^3$ patch. These plane partitions are identified with melted crystal configurations, and then topological vertex gluing rules may be understood as a prescription for composing together such crystals. In principle this allows to interpret the whole class of toric manifolds discussed in section \ref{ssec-toric} in a crystal language, however their gluing does not have any obvious three-dimensional interpretation.
 
Secondly, there is another class of crystal models which do have a straightforward three-dimensional interpretation, even though they are known only in a few particular cases and are not related explicitly to topological vertex gluing rules. In these models the entire crystal can be thought of as a container of a non-trivial shape, such that its melted configurations are in one-to-one correspondence with plane partitions. From this perspective the class of allowed plane partitions is of course restricted as they must fit into the container. A particular shape of the container is related to the Calabi-Yau target space geometry, and parameters determining the shape of the container correspond to K\"ahler moduli of this target space. In this thesis we mainly focus on this latter class of Calabi-Yau crystals. 

Calabi-Yau crystals also encode much more interesting information. On one hand, crystal generating functions which coincide with topological amplitudes turn out to encode Gopakumar-Vafa invariants in a very explicit way. On the other hand, crystal models are known also for certain amplitudes with branes, and the connection between branes and Chern-Simons theory leads to a correspondence between crystal models and knot invariants. We discuss all these intricaces in what follows. 

%?????????? The above mentioned relations are certainly not all reasons which make Calabi-Yau crystals a fascinating subject. Nonetheless, we do not know everything about them yet. In particular at present a general derivation what crystal model, or for example what shape of a container, should arise for a given Calabi-Yau manifold is not known. There are rather several cases of the correspondence known explicitly, which are the main subject of this thesis.  However, there are also some general indications that the relation to crystals should be more universal, which we also discuss in what follows. 

In the next section we explain what plane partitions are and in what sense they provide models of crystal melting. In the following sections in this chapter we introduce other aspects of crystal models: interpretation of crystals as quantum Calabi-Yau manifolds, relation to the topological vertex and branes. In the next chapter we will introduce and analyze models of the second type mentioned above.

 

==> partition-3d.tex <==
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.4\textwidth]{crystal-3d-xyz.eps}
\includegraphics[width=0.4\textwidth]{crystal-3d-2d-xyz.eps}
\caption{Plane partition (left) and its presentation in terms of interlacing Young diagrams (right). This plane partition represents a particular configuration of a crystal which initially (before melting) entirely filled a positive octant of $\Z^3$. It is understood all boxes (atoms) this plane partition consists of have melted away, and remaining non-melted atoms (not drawn) remain in their original positions. As discussed in the text, a unit distance along each direction is measured in $g_s$ units from topological strings point of view.} \label{fig-crystal3d}
\end{center}
\end{figure}

\section{Plane partitions}

We wish to consider statistical models of crystal melting. In these models it is assumed a crystal consists of atoms represented by unit boxes located in integer points of a three-dimensional lattice which is some subset of $\Z^3$, and melting can be localized only in a neighbouhood of crystal corners. This lattice can be thought of as a container initially filled entirely with atoms, which depart from the crystal in the process of melting. A given melted configuration of the crystal, with some places vacant due to melted atoms, can be assigned a statistical weight defined by the number of melted atoms. Denoting such a configuration by $\pi$ and a number of vacant boxes it contains by $|\pi|$, the partition or generating function of this system reads
\be
Z=\sum_{\pi}q^{|\pi|},           \label{generating}
\ee
where $q=e^{-\mu/T}$ is related to a chemical potential $\mu$ and temperature $T$ from the statistical point of view. In general the crystal begins to melt in large temperature, and in $T\to\infty$ limit it aproaches a limit shape which can be identified after rescaling the container in all directions by a factor $1/T$. The simplest crystal model of this type involves a lattice which is just a positive octant of $\Z^3$, and more complicated models can be thought of as modifications of this case. The configurations of melted atoms can be identified from mathematical point of view with \emph{plane partitions} which we now introduce. 

Plane partitions are intimately related to two-dimensional parititions or Young diagrams, which on the other hand are in one-to-one correspondence with states of free fermions in two dimensions. Moreover, the correspondence with free fermions allows to find crystal partition functions in a very elegenat way in the so-called \emph{transfer matrix formalism}. Young diagrams and free fermions are introduced in appendix \ref{sec-partitions} where also their properties, which we use to large extent in what follows, are discussed in detail. All the notation below related to Young diagrams and free fermions is defined in that appendix.

A \emph{plane partition} (or three-dimensional partition) $\pi$ of shape $R$ is defined as a map from two-dimensional partition $R$ into positive integers
$$
\pi:\ R \longrightarrow \Z_+
$$
such that $\pi(m_1,n_1)\geq \pi(m_2,n_2)$ if $m_1\leq m_2$ and $n_1\leq n_2$. One can think of such a partition as a stack of boxes in a positive octant of $\Z^3$. Then the weight of $\pi$ is given as the total number of these boxes
$$
|\pi| = \sum_{(m,n)\in R} \pi(m,n).
$$
This is an example of a plane partition of shape $R=(5,3,3,1)$ 
$$
\pi = \left( \begin{array}{ccccc} 5 & 3 & 2 & 1 & 1  \\
3 & 2 & 1 & & \\
2 & 1 & 1 & & \\
1 &   &   & & \\
\end{array} \right)
$$
presented also in figure \ref{fig-crystal3d}. In this case the weight is $|\pi| = 23$. 

These plane partitions may be thought of as configurations of an infinite crystal identified with a positive octant of $\Z^3$ lattice. However, one can impose some additional constraints, for example by restricting to a subset of this octant. In this thesis we are interested in generating functions of various such ensambles of plane partitions. %Free fermion formalism is a very useful tool for computation of these generating functions. 

We focus now on a prototypical and the simplest example of crystal melting, which is represented by plane partitions contained in the positive octant of $\Z^3$ introduced above, without any further constraints. This case provides also an example of the transfer matrix formalism.

To start with, let us notice any plane partition can be presented as a set of Young diagrams $\pi(t)$ obtained from a diagonal slicing of $\Z^3$ by planes $y=x-t$ with $t\in\Z$. A definition of $x,y,z$ axes together with an example of such slicing is shown in figure \ref{fig-crystal3d}. The crucial observation is these Young diagrams interlace (\ref{interlace}) each other
$$
\ldots \prec \pi(-3) \prec \pi(-2) \prec \pi(-1) \prec \pi(0) \succ \pi(1) \succ \pi(2) \succ \pi(3) \succ \ldots.
$$
Thus all possible plane partitions can be built from the charge $p=0$ vacuum using a string of vertex operators (\ref{gamma-1-build}). Let $q$ denote a weight of a single box in a plane partition $\pi$. To weight $\pi$ appropriately we note
$$
q^{|\pi|} = q^{\sum_{t\in\Z} |\pi(t)|},
$$
so due to the property (\ref{L0}) it is enough to insert $q^{L_0}$ at each slice $t$. Using the commutation relation (\ref{commute}) and the property (\ref{gamma-z-1}) the generating function of all partitions can be computed as follows
\bea
M(q) & = & \sum_{\pi} q^{|\pi|} = \langle0| \Big(\prod_{t=0}^{\infty} q^{L_0} \G_+(1)\Big) q^{L_0} \Big(\prod_{t=-1}^{-\infty} \G_-(1) q^{L_0}  \Big) |0\rangle = \nonumber \\
& = & \langle 0|\prod_{n>0}\Gamma_{+}(q^{n-1/2})\,\prod_{m>0}\Gamma_{-}(q^{-(m-1/2)})|0\rangle = \nonumber \\
& = & \prod_{n,m>0}\Big(1-\frac{q^{n-1/2}}{q^{-m+1/2}}\Big)^{-1}=\prod_{k>0}(1-q^{k})^{-k} = e^{\sum_{k>0} \frac{1}{k[k]^2}}. \label{McMahon}
\eea
This generating function is denoted $M(q)$ and is called the McMahon function to honour a mathematician who found it. The expectation value in the first line is called a \emph{transfer matrix}, and its evaluation is an example of the \emph{transfer matrix formalism}.

In fact, McMahon derived also much more general generating function of plane
partitions restricted to lie inside a cube of size $M\times L\times N$. It is
given by formula (\ref{Z1Z2}) and we discuss it in detail in the context of
Calabi-Yau crystals in section \ref{sec-closed-ver}.





==> title-bis.tex <==
\newpage
\thispagestyle{empty}

\begin{center}
 \large Uniwersytet Warszawski \\
Wydzia{\l}   Fizyki\\
 Instytut Fizyki Teoretycznej
\vskip 1.5 cm


{\bf\Huge Calabi-Yau crystals \\ 
\vskip 10pt
\bf\Huge in topological string theory }

\vskip 10pt

{\bf \large{Kryszta\l y Calabi-Yau w topologicznej teorii strun}}\\
\vskip 1 cm

{\large{Rozprawa doktorska}} \\
\vskip 0.8 cm

\begin{center}
\epsfig{file=AGUILA.PS,width=5cm}
\end{center}
\vspace*{0.7cm}

{\bf \Huge{\emph{ Piotr Su\l kowski }}}\\
\vskip 1.0cm

{\large{Promotorzy:}} \\

\vskip 0.2 cm
%{{\bf Prof. dr Robbert Dijkgraaf,} $\quad$  {\bf dr hab. Jacek Pawe\l czyk, prof UW}}
{\bf \large{Prof. dr Robbert Dijkgraaf}} \\
{\bf \large{dr hab. Jacek Pawe\l czyk, prof. UW }}


%\begin{center}
%Zak"lad Teorii Cz"astek Elementarnych \\ i Oddzia"lywa"n Fundamentalnych
%\end{center}
\vskip 1.0 cm
\begin{center}
{\large Warszawa, Czerwiec 2007}
\end{center}
\end{center}
\newpage 
\thispagestyle{empty}
{\tiny{{.}}}


\newpage
\thispagestyle{empty}
{\tiny{{.}}}
\vskip 18cm

\begin{flushright}
{\bf \huge{\emph{Całej mojej rodzinie  }}}\\
\end{flushright}




